Improving Multi-turn Emotional Support Dialogue Generation with Lookahead Strategy Planning

Providing Emotional Support (ES) to soothe people in emotional distress is an essential capability in social interactions. Most existing researches on building ES conversation systems only considered single-turn interactions with users, which was over-simplified. In comparison, multi-turn ES conversation systems can provide ES more effectively, but face several new technical challenges, including: (1) how to adopt appropriate support strategies to achieve the long-term dialogue goal of comforting the user's emotion; (2) how to dynamically model the user's state. In this paper, we propose a novel system MultiESC to address these issues. For strategy planning, drawing inspiration from the A* search algorithm, we propose lookahead heuristics to estimate the future user feedback after using particular strategies, which helps to select strategies that can lead to the best long-term effects. For user state modeling, MultiESC focuses on capturing users' subtle emotional expressions and understanding their emotion causes. Extensive experiments show that MultiESC significantly outperforms competitive baselines in both dialogue generation and strategy planning. Our codes are available at https://github.com/lwgkzl/MultiESC.

==> Table/2_generation_human.tex <==
\begin{table}[t]
\small
    \centering\scalebox{0.95}{
    \begin{tabular}{l  l lcr }
        \specialrule{1.2pt}{1pt}{1pt}
        \textbf{MultiESC vs.} & {\textbf{Metrics}} & \textbf{Win} & \textbf{Lose}  & \textbf{Tie$\;$}\\
        \specialrule{1.0pt}{0.5pt}{0.5pt}
         \multirow{5}[0]{*}{{MoEL}} & {Fluency} & \textbf{64.1}$^{\ddag}$ & 18.0   & 18.0\\
        & {Empathy} &  \textbf{53.1}$^{\ddag}$  & 34.4  & 12.5 \\
        & {Identification} & \textbf{69.5}$^{\ddag}$  & 22.7   & 7.9\\
        & {Suggestion} &  \textbf{71.9}$^{\ddag}$  & 14.8   & 13.3\\
        %\specialrule{0.7pt}{0.5pt}{0.5pt}
        & {Overall} &  \textbf{65.6}$^{\ddag}$  & 20.3  & 14.1\\\specialrule{0.7pt}{0.5pt}{0.5pt}
        \multirow{5}[0]{*}{{BlenderBot-Joint}} & {Fluency} & 35.2 & \textbf{42.9} & 21.9 \\
        & {Empathy} & \textbf{44.5} & 43.8   & 11.7 \\
        & {Identification} &  \textbf{48.4}$^{\ddag}$  & 32.8 & 18.8  \\
        & {Suggestion} &  \textbf{60.9}$^{\ddag}$  & 23.4  & 15.6 \\
        %\specialrule{0.7pt}{0.5pt}{0.5pt}
        & {Overall} &  \textbf{58.6}$^{\ddag}$  & 31.3 & 10.2 \\\specialrule{0.7pt}{0.5pt}{0.5pt}
        \multirow{5}[0]{*}{{\emph{w/o} strategy}} & {Fluency}  & 38.3 & \textbf{41.4} & 20.3\\
        & {Empathy} & \textbf{43.8}$^{\dag}$ & 29.7  & 26.5 \\
        & {Identification} &  \textbf{56.3}$^{\ddag}$  & 32.8 & 10.9  \\
        & {Suggestion} &  \textbf{52.3}$^{\dag}$  & 36.7  & 10.9 \\
        %\specialrule{0.7pt}{0.5pt}{0.5pt}
        & {Overall} &  \textbf{55.5}$^{\ddag}$  & 30.5 & 14.0 \\\specialrule{0.7pt}{0.5pt}{0.5pt}
        \multirow{5}[0]{*}{{\emph{w/o} lookahead}} & {Fluency} &  \textbf{41.4}  & 37.5 & 21.1 \\
        & {Empathy} &  35.9  & \textbf{39.1} & 25.0 \\
        & {Identification} & \textbf{46.9}$^{\ddag}$  & 28.9 & 14.2 \\
        & {Suggestion} & \textbf{44.5}$^{\dag}$  & 30.5 & 25.0 \\
        %\specialrule{0.7pt}{0.5pt}{0.5pt}
        & {Overall} & \textbf{46.1}$^{\dag}$  & 32.0 & 21.9 \\
        \specialrule{1.2pt}{0.5pt}{0pt}
    \end{tabular}}%
    \caption{Human interactive evaluation results (\%). ${\dag} / {\ddag}$ denote $p$-value $< 0.1 / 0.05$ (statistical significance test).}
    %\vspace{-15mm}
    \label{tbl:generation_human}
\end{table}

==> Table/5_user_state_modeling.tex <==
\begin{table}[t]
\small
\centering
	\begin{center}
		\begin{tabular}{ l  ccccc } \specialrule{1.0pt}{1pt}{1pt}
        \small{\textbf{Model}} & \small{\textbf{B-1}} & \small{\textbf{B-2}} & \small{\textbf{R-L}} & \textbf{MET} & \small{\textbf{CID}$\;$} \\ \specialrule{1.0pt}{0pt}{0.5pt}
        \textsc{MultiESC}  & \textbf{21.81} & \textbf{9.36}  & \textbf{20.23} & \textbf{8.79} & \textbf{31.16} \\
        \emph{w/o} cause & 20.07 & 8.42 &19.99  &8.24  &27.25 \\ 
        \emph{w/o} emotion & 19.21 & 8.27 & 20.70 & 8.31 & 28.43 \\
        \emph{w/o} strategy  & 20.67 & 8.91  & 19.79 & 8.47 & 28.93 \\
        \emph{w/o} lookahead \\\specialrule{1.0pt}{0.5pt}{0pt}
		\end{tabular}
	\end{center}
	\caption{The results of ablation study on the components of MultiESC.}
\label{tbl:user_state}
\end{table}

==> Table/6_strategy_distribution.tex <==
\begin{table}[t]%BLUE1 BLEU2也可以删掉
\small
	\begin{center}
		\begin{tabular}{ l  c c c c c} \specialrule{1.0pt}{1pt}{1pt}
        \small{\textbf{Model}} & \small{\textbf{S-1}} &  \small{\textbf{S-2}} & \small{\textbf{S-3}}  & \small{\textbf{S-4}} &  \small{\textbf{S-5}}\\ \specialrule{1.0pt}{0pt}{0.5pt} 
        BERT &  \\
        %Bart &  38.34 & 27.97 \\
         HED & \\
         Sequicity\\
         DialogGPT\\
         BlenderBot\\
         \specialrule{0.7pt}{0.5pt}{0.5pt}
        Ours  \\
        \emph{w/o} lookahead \\
        % \emph{OUR} & 40.07 & 28.90\\
         \specialrule{1.0pt}{0.5pt}{0pt}
         
        %Ours$_{\rm 1\text{-}hop}$ & 16.23 & 20.25 & 31.27 \\ \hline 
		\end{tabular}
	\end{center}
	\caption{Strategy distribution of MultiESC and baselines at different conversation stages.}
\label{tbl:strategy_acc}
\end{table}

==> backup/3_Methodology.tex <==
\section{Methodology}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figure/fig_overall architecture.pdf}
    \caption{The overall framework of \textsc{MultiESC}. More details about the user state modeling and the strategy planning modules are shown in Figure \ref{fig:user_state_modeling} and \ref{fig:strategy_planning}.}
    \label{fig:overall_architecture}
\end{figure}



%\subsection{Method Overview}
%In a multi-turn emotional support conversation, the user is in a depressed emotional state and the supporter (or the system) aims to lower the intensity of the user's emotional distress through interactions. 
We denote the dialogue context before the $t$-th conversation round as $D_{t}$=$\{(x_i, y_i)\}_{i=1}^{t-1}$, an alternating set of utterances between the system and the user; $U_t = \{u_1,u_2,..., u_{t-1}\}$ represent the set of user states at the history dialogue turns. 
Our system aims to track the user state $U_t$ from the dialogue context $D_t$ and generates an utterance $x_{t}$, using an appropriate support strategy $s_{t}$. 
We denote the set of all possible strategies as $\mathbb{S}$. 

As shown in Figure \ref{fig:overall_architecture}, our proposed system, \textsc{MultiESC}, mainly consists of four modules. 
%, where $x_i, y_i$ are respectively the user's and the system's utterances at the $i$-th round. 
The \emph{dialogue encoder} module first converts  $D_{t}$ into the dialogue history embeddings $H_t$, while the \emph{user state modeling} module is implemented to identify the user state information $U_t$ from $D_{t}$.
Then, the \emph{strategy planning} module selects the strategy $s_t$ based on $H_t$ and $U_t$. 
Finally, the \emph{utterance decoder} produces the utterance $x_t$, using the strategy $s_{t}$. 
%To generate the utterance $x_t$ \blue{maybe yt }, \textsc{MultiESC} first models the current user state $u_{_t}$ given $\mathcal{H}_t$. Then, a strategy planning module selects the next strategy $s_{_t}$ to be adopted at this turn based on the user state $u_{_t}$. Finally, a strategy-enhanced generator produces the utterance $x_t$ that utilizes strategy $s_{_t}$. 
In what follows, we will introduce the four modules in more detail.

\subsection{Dialogue Encoder}
The dialogue encoder module is implemented with a Transformer encoder \cite{vaswani2017attention}. We concatenate the utterances in $D_{t}$ and keep the last $N$ tokens of the concatenation as its input sequence. 
Given the input, it produces the dialogue history embeddings $H_t$  $\in$ $\mathbb{R}^{N \times d_{\text{emb}}}$. 

\subsection{User State Modeling}

To obtain the local user state at each dialogue turn, we first identify the emotion causes $c_i$ mentioned at the $i$-th turn with an off-the-shelf tool for emotion cause detection, which is trained on a large open-domain dataset \cite{poria2021recognizing}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figure/fig_user state modeling.pdf}
    \caption{The user state modeling module in  \textsc{MultiESC}.}
    \label{fig:user_state_modeling}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{Figure/fig_strategy planning.pdf}
    \caption{The process of calculating the strategy score $\mathbf{F}(s_t)$, with a strategy sequence generator and a user feedback predictor. }%Illustration of the strategy planning module in  \textsc{MultiESC}. It selects the next strategy that maximizes the score of $F(s_t)$.}
    \label{fig:strategy_planning}
\end{figure*}

Then, an emotion-aware Transformer encoder is utilized to obtain the local user state embedding $u_i$. 
Specifically, the special tokens [CLS], [SEP] and [EC] are respectively inserted at the beginning of $x_i$, $y_i$ and $c_i$ to form the input sequence. $x_i$ is also considered because the supporter's utterance often provides necessary context for understanding the user state. 
To fuse the emotion information, we incorporate emotion embeddings $E_{e}$ in the input representation. Specifically, we use the positional sum of the emotion embeddings $E_{e}$, the word embeddings $E_{w}$ and the positional embeddings $E_{w}$ to represent the input sequence. 

In our work, we train multiple emotion vectors ${e_1, e_2, ..., e_{n_{emo}}}$ to represent different emotional states. To obtain the emotion embeddings $E_{e}$ for a given input sequence, we concatenate the emotion vector corresponding to the emotional state of each word in the input sequence.  
Concretely, we split the VAD space into $n_{V} \cdot n_{A}$ subspaces by dividing the valence and the arousal dimensions, respectively, into $n_{V}$ and $n_{A}$ intervals of equal length. Each trainable emotion vector is maintained to represent the emotional states in one of the subspaces. Thus, there are overall $n_{emo} = n_{V} \cdot n_{A}$ types of emotion embeddings.
 \footnote{The dominance dimension is not considered here as it is less relevant for capturing emotion intensity \cite{zhong2019knowledge}. } 
Given the input sequence, we find the corresponding emotion vector of each token based on its VAD scores annotated in the NRC\_VAD lexicon. For those tokens without VAD annotation, we use the average of all the emotion vectors as its emotion embedding. 


Finally, the encoded hidden state corresponding to the [CLS] token is used to represent the local user state embedding $u_i$ at the $i$-th turn. We denote the concatenation of all the user state embeddings before the $t$-th turns as $U_t$=$[u_1; u_2;...;u_{t-1}]$.



%\cite{park2021dimensional}





\subsection{Strategy Planning with Lookahead Heuristics}
In the section, we will first introduce a standard scheme of dialogue strategy selection, which is purely history-based without foresight of the strategy long-term effect. 
Then, we will analyze its shortcomings and how it can be improved by incorporating our proposed lookahead heuristics. 
Finally, we will describe how we concretely realize the strategy inference in \textsc{MultiESC}. 

\subsubsection{History-based Strategy Selection} 
A standard scheme of dialogue strategy selection is to compute the conditional probability distribution of the next strategy given the current user state. This computation can be learned by using the ground-truth label of the next strategy as supervision. A each round, it selects the strategy that maximizes 
\begin{equation}
    g(s_{_t})=-\log P(s_{_t}|u_{_t}).\label{eq:g(s_{_t})}
\end{equation}
However, such scheme is purely history-based, lacking foresight of the strategy's long-term effect and how much it could help in achieving the goal of comforting the user's emotional distress. 
Though previous researches on dialogue strategy planning may have varied in their methods of modeling the dialogue history and obtaining $u_t$, they generally followed this history-based scheme \cite{zhou2019augmenting, joshi2021dialograph, dutt2021resper}.

\subsubsection{Incorporating Lookahead Heuristics}
To address the above issue, we draw inspiration from the classical search algorithm, $\text{A}^{*}$ search \cite{hart1968formal}, which searches the highest-scoring path by selecting actions that maximize $\hat{F}(a)$=$\hat{g}(a) + \hat{h}(a)$, where $\hat{g}(a)$ is the score-so-far and $\hat{h}(a)$ is a heuristic estimation of the future score. In our work, we select the next strategy $s_{_t}$ that maximizes
\begin{equation}
    F(s_{_t}) = g(s_{_t})+\lambda\cdot h(s_{_t}),\label{eq:F(s_{_t})}
\end{equation}
where $\lambda$ is a hyper-parameter and $g(s_{_t})$ is a purely history-based strategy prediction score computed as in Equation \ref{eq:g(s_{_t})}; 
$h(s_{_t})$ is the lookahead heuristic that estimates \emph{the expectation of future user feedback} (a score indicating indicating how much the user's emotional distress is reduced). Ideally, $h(s_{_t})$ should be computed as
\begin{align}
    h(s_{_t}) &= \text{E}[f(u_{_t},s_{_t},s_{_{>t}})|s_{_t},u_{_t}]\nonumber\\
    &=\sum_{s_{_{>t}}\in \mathbf{S}}P(s_{_{>t}}|s_{_t},u_{_t})\cdot f(u_{_t},s_{_t},s_{_{>t}}).  \label{eq:perfect_h(s_t)}
\end{align}
In Equation \ref{eq:perfect_h(s_t)}, $s_{_{>t}}$ represents the strategy sequence to be used after the $t$-th turn till the end of the conversation. $\mathbf{S}$ is the set of all strategy sequences. The function $f(u_{_t},s_{_t},s_{_{>t}})$ denotes the user feedback score at the end of the conversation, if the strategies $s_{_t},s_{_{>t}}$ are used to comfort a user whose state is $u_t$.\footnote{Here, we assume that how much the user's emotion intensity decreases after the conversation is only affected by the strategies adopted by the supporter, neglecting the specific content of the supporter's utterances (i.e., hypothesizing the supporter could always utter the most appropriate content that adopts the given strategy). }
However, two difficulties arises in calculating Equation \ref{eq:perfect_h(s_t)}: (1) the space of $\mathbf{S}$ is too large; (2) it is difficult to compute the user feedback $f(\cdot)$ after a long strategy sequence. 

Thus, we can approximate the above equation by narrowing the space of $\mathbf{S}$ to part of the strategy sequences with limited length. Specifically, Equation \ref{eq:perfect_h(s_t)} is approximated as
\begin{align}
    h(s_{_t}) &= \sum_{s_{_{>t}}\in \mathbf{\hat{S}}_{_L}}P(s_{_{>t}}|s_{_t},u_{_t})\cdot f(u_{_t},s_{_{\geq t}}), \label{eq:h(s_{_t})}\\
    \mathbf{\hat{S}}_{_{L}} &= \argtopk_{s_{_{>t}}\in \mathbf{S}_{_{L}}}P(s_{_{>t}}|s_{_t},u_{_t}),\label{eq:s_{_t}+1:t+L}
\end{align}
where $\mathbf{S}_{_{L}}$ is the set of strategy sequences whose lengths are less than $L$. 
%where $\mathbf{\hat{S}}_{_{t+1:t+L}}$ is a subset of $\mathbf{S}_{_{t+1:t+L}}$ that satisfies

\subsubsection{Strategy Inference in MultiESC}
\label{sec:strategyMultiESC}
As shown in Figure \ref{fig:strategy_planning}, two components in \textsc{Multi-ESC} are jointly responsible for obtaining the score $F(s_{_t})$ for each possible strategy, i.e., a strategy sequence generator and a user feedback predictor. %Figure \ref{fig:strategy_planning} shows their architecture and how we leverage them to calculate the strategy score during inference. 
In the following, we will first describe their architectures respectively and then illustrate how we leverage them to calculate the strategy score during inference. 

\paragraph{Strategy Sequence Generator (SSG)}  
Given the current user state $U_{_t}$ and the the dialogue history $H_{t}$, this component aims to sequentially predict the strategy sequence $s_{_{t:t+L}}$ that will be used in the following $L$ turns. 
As shown in Figure \ref{fig:strategy_planning}, it is developed upon the Transformer decoder architecture \cite{vaswani2017attention}, with a multi-source attention mechanism to selectively focus on the both the dialogue history and the user state information. 

The shifted right strategy sequence is first fed to a masked multi-head attention layer, followed by add and normalization, producing the contextualized strategy sequence representations $\mathbf{P}_t$. 
Then, $\mathbf{P}_t$ interacts with the dialogue history embeddings $\mathbf{H}_t$ and the user state embeddings $\mathbf{U}_t$, respectively, through cross attention layers as follows:
\begin{align}
    \hat{\mathbf{H}}_t &= \text{MH}(L(\mathbf{P}_t), L(\mathbf{H}_t), L(\mathbf{H}_t)),\\
    \hat{\mathbf{U}}_t &= \text{MH}(L(\mathbf{P}_t), L(\mathbf{U}_t), L(\mathbf{U}_t)),
\end{align}
where $L$($\cdot$) linearly transforms embeddings to form $h$ heads and MH($\cdot$) stands for the multi-headed self-attention mechanism.  
An information fusion layer is utilized to combine $\hat{\mathbf{H}}_t$ and $\hat{\mathbf{U}}_t$ as below:
\begin{align}
    \mu &= \text{sigmoid}(\mathbf{W}_{\mu}[\hat{\mathbf{H}}_t; \hat{\mathbf{U}}_t]+\mathbf{b}_{\mu}), \\
    \hat{\mathbf{P}}_t  &= \mu \cdot \hat{\mathbf{H}}_t + (1-\mu) \cdot  \hat{\mathbf{U}}_t. 
\end{align}
where $\mathbf{W}_{\mu}$ and $\mathbf{b}_{\mu}$ are trainable parameters. 

Next, $\hat{\mathbf{P}}_t$ is fed to a connected feed-forward network with a residual connection around the sub-layers, followed by layer normalization. Denoting the resulted representations as $\widetilde{\mathbf{P}}_t$, the generator yields the distribution over strategies at the timestep $l$ ($l$=0,1,..,$L$-1):
\begin{equation}
    P(s_{_{t+l}}|s_{_{t:t+l}}, \mathbf{H}_t, \mathbf{U}_t)=\text{softmax}(\mathbf{W}_s\widetilde{\mathbf{P}}_t+\mathbf{b}_s)\nonumber
\end{equation}
where $\mathbf{W}_{s}$ and $\mathbf{b}_{s}$ are trainable parameters.

For training of the strategy sequence generator, we use the negative log-likelihood of the ground-truth strategy $s_{_{t+l}}^{*}$ as its loss function:
\begin{align}
  \mathcal{L}_{s} &= -\sum_{l=
  0}^{L-1} \log P(s_{_{t+l}}=s_{_{t+l}}^{*}\mid s_{_{t:t+l}}^{*}, \mathbf{H}_t, \mathbf{U}_t).\nonumber
\end{align}

\paragraph{User Feedback Predictor (UFP)} This component aims to estimate the user feedback $f(u_{_t}, s_{_{t:t+L}})$ after the system adopts the strategy sequence $s_{_{t:t+L}}$ in the following turns, given the previous user sates $\{u_1,u_2,..,u_{t-1}\}$. 
It is develop based upon the Transformer encoder. 
The input sequence is the concatenation of the previous user states and the following strategy sequence; the special token [SEP] is inserted between them and [CLS] at the very beginning. 
The user states are represented with the user state embeddings $\mathbf{U}_t$, while we leverage trainable strategy embeddings $\mathbf{E}_s \in \mathbb{R}^{|\mathbb{S}| \times d_{\text{emb}}}$ to represent each strategy embedding. Denoting the Transformer Encoder as $\text{TRS}_{\text{Enc}}$, then we have the resulted representations:
\begin{equation}
    \mathbf{B} = \text{TRS}_{\text{Enc}}[\text{Emb}(\text{[CLS]}; u_{1:t-1};\text{[SEP]};s_{t:t+L})],\nonumber
\end{equation}
where Emb($\cdot$) represent the conversion operation of the embedding layer, and $\mathbf{B} \in \mathbb{R}^{(t+L+1)\times d_{emb}}$. 
Then, we define the encoded hidden state corresponding to the [CLS] token as $\mathbf{q}_f=\mathbf{B}_0$, which is used to calculate the user feedback score through a feedforward layer:
\begin{align}
    f(u_{_t}, s_{_{t:t+L}}) = \mathbf{W}_f\mathbf{q}_f+\mathbf{b}_f\nonumber
\end{align}
where $\mathbf{W}_{f}$ and $\mathbf{b}_{f}$ are trainable parameters. 

As ground-truth user feedback scores are provided in the \textsc{ESConv} datasets, our user feedback predictor can thus be trained through supervised learning . We use the Mean Square Error (MSE) as its loss function $\mathcal{L}_{f}$. %For training of the user feedback predictor, the negative log-likelihood of the ground-truth strategy $s_{_{t+l}}^{*}$ as its loss function:

\paragraph{Strategy Score Calculation} 
Figure \ref{fig:strategy_planning} presents the process of calculating strategy scores during inference. 
We first use SSG to derive the probability of the next strategy $P(s_{_t}|,\mathbf{U}_{_t}, ,\mathbf{H}_{_t})$, and thus obtain the history-based score $g(s_{_t})$. Note that we can also use SSG to further compute the probability of the remaining strategy sequence $s_{_{t+1:t+L}}$ as:
\begin{equation}
    \resizebox{\hsize}{!}{$P(s_{_{t+1:t+L}}|s_{_t},\mathbf{U}_{_t},\mathbf{H}_{_t})=\prod_{l=1}^{L-1} P(s_{_{t+l}}|s_{_{t:t+l}},\mathbf{U}_{_t},\mathbf{H}_{_t})$}\nonumber
\end{equation}
To calculate the lookahead score $h(s_{_t})$, we leverage SSG to find the set of most possible future strategy sequences $\mathbf{\hat{S}}_{_{L}}$ in Equation \ref{eq:s_{_t}+1:t+L} through beam search. 
Then, we calculate the their probabilities and the estimated user feedback after using them, respectively with SSG and UFP, which are then used to compute  $h(s_{_t})$ as in Equation \ref{eq:h(s_{_t})}. 
Finally, given $g(s_{_t})$ and $h(s_{_t})$, the strategy score is obtained as in Equation \ref{eq:F(s_{_t})}.

\subsection{Utterance Decoder} 
Given the user state embeddings $\mathbf{U}_{_t}$, the history embeddings $\mathbf{H}_t$, and the selected strategy $s_{_t}$, the utterance decoder aims to produce the next utterance $x_{t}$. 
It is developed upon the backbone of the Transformer decoder. 
Its architecture is similar to that of the strategy sequence generator as shown in Figure \ref{fig:strategy_planning}, except for the input sequence. 
To guide the generation with the selected strategy $s_{_t}$, we concatenate the strategy embedding of $s_{_t}$ with the embeddings of the shifted right response sequence as the input of the utterance decoder. The negative likelihood of the ground-truth token in the target utterance is used as the generation loss $\mathcal{L}_{g}$. 

%\cite{liu2021pre}

==> backup/3_Methodology_2.0.tex <==
\section{Methodology}

As shown in Fig. \ref{fig:overall_architecture}, our proposed system  \textsc{MultiESC} consists of four modules. 
The dialogue encoder first converts  the dialogue history $\mathcal{H}_{t}$ into the embeddings $\mathbf{H}_t$. At the same time,  the user state modeling module extracts the user state information, producing the embeddings $\mathbf{U}_t$.
Then, given $\mathbf{H}_t$ and $\mathbf{U}_t$, the strategy planning module selects the support strategy $s_t$ . 
Finally, the utterance decoder generates the utterance $x_t$ that adopts the strategy $s_{t}$. 
%To generate the utterance $x_t$ \blue{maybe yt }, \textsc{MultiESC} first models the current user state $u_{t}$ given $\mathcal{H}_t$. Then, a strategy planning module selects the next strategy $s_{t}$ to be adopted at this turn based on the user state $u_{t}$. Finally, a strategy-enhanced generator produces the utterance $x_t$ that utilizes strategy $s_{t}$. 
In what follows, we will introduce the four modules in more detail.

\subsection{Dialogue Encoder}
The dialogue encoder module is implemented with a Transformer encoder \cite{vaswani2017attention}. We concatenate the utterances in $\mathcal{H}_{t}$ and keep the last $N$ tokens of the concatenation as its input sequence. 
Given the input, it produces the dialogue history embeddings $\mathbf{H}_t$  $\in$ $\mathbb{R}^{N \times d_{\text{emb}}}$. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figure/fig_user state modeling.pdf}
    \caption{The architecture of the user state modeling module in \textsc{MultiESC}.}
    \label{fig:user_state_modeling}
\end{figure}

\subsection{User State Modeling}

%For user state modeling, we mainly focus on two aspects: the user's \emph{emotional state} and \emph{emotion causes}. 
Fig. \ref{fig:user_state_modeling} illustrates the workflow of user state modeling. 
To identify the user's state at the $i$-th round of the conversation, we first extract the emotion causes mentioned at this round with an off-the-shelf detector\footnote{\url{https://github.com/declare-lab/RECCON}}, which is trained on a large-scale emotion cause detection dataset \cite{poria2021recognizing}. 

Then, we concatenate the dialogue content $x_i$, $y_i$ and the emotion causes $c_i$ as the input of a Transformer encoder. Special tokens are inserted to separate different segments. The system's utterance $x_i$ is also considered because it often provides necessary context for understanding the user's state. 
The input sequence is represented as the positional sum of \emph{emotion embeddings}, word embeddings, and positional embeddings. 
The emotion embeddings are used to fuse the emotion information. They are obtained as follows.  
We train multiple emotion vectors $\{\mathbf{e}_1, \mathbf{e}_2, ..., \mathbf{e}_{n_{\text{emo}}}\}$ to represent the underlying emotions of different words. 
%To obtain the emotion embeddings $\mathbf{E}_{e}$ for a given input sequence, we concatenate the emotion vector corresponding to the emotion intensity of each word in the input sequence.  
Concretely, we split the VAD space into multiple subspaces by dividing the valence and the arousal dimensions, respectively, into $n_{\text{V}}$ and $n_{\text{A}}$ intervals of equal length. 
Each emotional subspace is represented as one emotion vector $e_j$ represent.\footnote{The dominance dimension is not considered here as it is less relevant for capturing emotion intensity \cite{zhong2019knowledge,li2020knowledge}.} 
To construct the emotion embeddings, we retrieve the VAD score of each input token from the NRC\_VAD lexicon to identify which emotional subspace it belongs, and then we represent it as the corresponding emotion vector.  %and map them to their corresponding emotion vectors, which are then concatenated in the emotion embedding layer. %be part of the input representation. 
For those tokens without VAD annotation, we use a special emotion vector to represent them. %Thus, the number of the emotion vectors $n_{\text{emo}}$ is $n_{\text{V}}\cdot n_{\text{A}}+1$. 


Finally, the encoded hidden vector $\mathbf{u}_i$  corresponding to the $\texttt{[CLS]}$ token is used to represent the user state at the $i$-th round. The user state embeddings $\mathbf{U}_t$ is the concatenation of all the user state embeddings before the $t$-th round, that is, $\mathbf{U}_t$=$[\mathbf{u}_1; \mathbf{u}_2;...;\mathbf{u}_{t-1}]$.

%\cite{park2021dimensional}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{Figure/fig_strategy planning.pdf}
    \caption{The process of calculating the strategy score, using a strategy sequence generator and a user feedback predictor. At each turn, our model selects the next strategy that maximizes the score of $F(s_t)$. }%Illustration of the strategy planning module in  \textsc{MultiESC}. It selects the next strategy that maximizes the score of $F(s_t)$.}
    \label{fig:strategy_planning}
\end{figure*}

\subsection{Feedback-oriented Strategy Planning with Lookahead Heuristics}
In the section, we will first introduce a standard scheme of dialogue strategy selection, which is purely history-based without foresight on a long planning horizon. 
Then, we will analyze its shortcomings and how it can be improved by incorporating our proposed lookahead heuristics. 
Finally, we will describe how we concretely realize the strategy inference in \textsc{MultiESC}. 

\subsubsection{Strategy Score} 
\paragraph{History-based Score}
A standard scheme of dialogue strategy selection is to compute the conditional probability distribution of the next strategy purely based on the dialogue history and the previous user states. 
%This computation can be learned by using the ground-truth label of the next strategy as supervision. 
In other words, at each round, it selects the strategy that maximizes: 
\begin{equation}
    g(s_{t})=-\log \text{Pr}(s_{t}|\mathbf{H}_{t}, \mathbf{U}_{t}).\label{eq:g(s_{t})}
\end{equation}
Though previous researches on dialogue strategy planning may have varied in their methods of obtaining representation of the dialogue history $\mathbf{H}_{t}$ and the one of the user states $\mathbf{U}_{t}$, they generally followed this history-based scheme \cite{zhou2019augmenting, joshi2021dialograph, dutt2021resper}. However, such practice overlooked the strategy's long-term effect and how much it could help in achieving the final goal of comforting the user's emotional distress. 

\paragraph{Lookahead Score}
To address the above issue, we propose a method that incorporates lookahead planning with consideration of the future user feedback. 
Our method draws inspiration from the classical search algorithm, $\text{A}^{*}$ search \cite{hart1968formal}, which conducts lookahead planning in a heuristic way. 
Specifically, it searches the highest-scoring path by selecting an action $a$ that maximize ${F}(a)={g}(a) + {h}(a)$ at each step, where ${g}(a)$ is the score-so-far and ${h}(a)$ is a heuristic estimation of the future score. 
In our work, we select the next strategy $s_{t}$ that maximizes the overall score $F(s_{t})$, which is defined as:
\begin{equation}
    F(s_{t}) = g(s_{t})+\lambda\cdot h(s_{t}).\label{eq:F(s_{t})}
\end{equation}
$g(s_{t})$ is a purely history-based strategy prediction score computed as in Eq. \ref{eq:g(s_{t})}, while $h(s_{t})$ heuristically estimates \emph{the mathematical expectation of future user feedback}. $\lambda$ is a hyper-parameter that balances the weights of the two terms. 

For the estimation of $h(s_{t})$, we only consider how much the adopted strategies would affect the user's emotion intensity and neglect the effects of other factors, such as the specific content of the utterances. % (i.e., hypothesizing the supporter could always utter the most appropriate content after selecting a correct strategy). 
Ideally, to select the strategy that achieves the best final results, we want to obtain the user feedback at the end of the conversation, which is computed as:
\begin{equation}
\resizebox{\hsize}{!}{$
    \begin{aligned}
        h(s_{t}) &= \text{E}[f(s_{t},s_{{>t}}, \mathbf{U}_{t})|s_{t},\mathbf{H}_t,\mathbf{U}_t]\\
        &=\sum_{s_{_{>t}}\in \mathcal{S}^{\omega}}\text{Pr}(s_{{>t}}|s_{t},\mathbf{H}_t,\mathbf{U}_t)\cdot f(s_{t},s_{{>t}},\mathbf{U}_t). 
    \end{aligned}\label{eq:perfect_h(s_t)}$}
\end{equation}
E($\cdot$) represents the mathematical expectation.  $s_{{>t}}$ is the strategy sequence to be used after the $t$-th turn till the end of the conversation.  
The function $f(s_{t},s_{>t}, \mathbf{U}_t)$ denotes the user feedback score after using strategies $s_{t},s_{{>t}}$ to comfort a user whose previous states are $\mathbf{U}_t$. 
$\mathcal{S}^{\omega}$ is the set of all possible strategy sequences, i.e., $\mathcal{S}^{\omega} = \bigcup_{n=0}^{\infty} \mathcal{S}^{n}$, where $\mathcal{S}^{n}$ is the $n$-ary Cartesian power the strategy set $\mathcal{S}$. 

However, two difficulties arises if we calculate $h(s_t)$ as in Eq. \ref{eq:perfect_h(s_t)}: (1) the space of $\mathcal{S}^{\omega}$ is too large; (2) it is difficult to compute the user feedback $f(\cdot)$ after too many turns (i.e. if the strategy sequence $s_{>t}$ is too long). 

To address the above challenges, we approximate Eq. \ref{eq:perfect_h(s_t)} by narrowing the space of strategy sequences $\mathcal{S}^{\omega}$. 
Specifically, we only consider strategy sequences whose lengths are less than $L$. We denote the set of strategy sequences whose lengths are less than $L$ is $\mathcal{S}_L$. %, instead of all the strategy sequences. 
Nevertheless, the space of $\mathcal{S}_L$, growing exponentially over the sequence length,  can still be too large. Thus, we further approximate the equation by only considering the $k$ most possible strategy sequences. 
Then, Eq. \ref{eq:perfect_h(s_t)} is approximated as: 
\begin{equation}
\resizebox{\hsize}{!}{$
    \begin{aligned}
        h(s_{t}) &= \sum_{s_{_{>t}}\in \mathbf{\hat{\mathcal{S}}}_{L}}\text{Pr}(s_{{>t}}|s_{t},\mathbf{H}_t,\mathbf{U}_{t})\cdot f(s_{t}, s_{>t}, \mathbf{U}_t), \\
        \mathbf{\hat{\mathcal{S}}}_{{L}} &= \argtopk_{s_{{>t}}\in \mathbf{S}_{{L}}}\text{Pr}(s_{{>t}}|s_{t},\mathbf{H}_t,\mathbf{U}_t).%\label{eq:s_{t}+1:t+L}
    \end{aligned}$}\label{eq:h(s_{t})}
\end{equation}

%where $\mathbf{\hat{S}}_{{t+1:t+L}}$ is a subset of $\mathbf{S}_{{t+1:t+L}}$ that satisfies

\subsubsection{Strategy Inference in MultiESC}
\label{sec:strategyMultiESC}
\vspace{1mm}\noindent\textbf{Process of Calculating Strategy Scores.} At each turn, \textsc{MultiESC} chooses to adopt the strategy that has the highest strategy score $F(s_t)$. 
As shown in Fig. \ref{fig:strategy_planning}, it calculates $F(s_t)$ with the help of two components: a Strategy Sequence Generator (SSG) and a User Feedback Predictor (UFP). 

The function of SSG is to sequentially predict $s_{\ge t}$, the strategy sequence that will be used in the following $L$ turns, based on $\mathbf{H}_{t}$ and $\mathbf{U}_{t}$. 
In other words, at the $l$-th timestep  ($l$=$0, 1, ..., L-1$), it outputs the predicted strategy distribution $\text{Pr}(s_{{t+l}}|s_{{t:t+l}},\textbf{H}_t,\textbf{U}_t)$. 
The function of UFP is to estimate the user feedback $f(s_{\ge t}, \mathbf{U}_t)$ after the system adopts the strategy sequence $s_{\ge t}$ to comfort the user, given the previous user sates $\mathbf{U}_{t}$. 

To calculate the overall strategy score $F(s_t)$, we first use SSG to derive the probability of the next strategy $\text{Pr}(s_{t}|\mathbf{H}_{t},\mathbf{U}_{t})$ and obtain the history-based score $g(s_{t})$ (Eq. \ref{eq:g(s_{t})}). 
Next, we use SSG to further compute the probability of the remaining strategy sequence $s_{>t}$ as:
\begin{equation}
    \resizebox{\hsize}{!}{$\text{Pr}(s_{>t}|s_{t},\mathbf{H}_{t}\mathbf{U}_{t})=\prod_{l=1}^{L-1} \text{Pr}(s_{{t+l}}|s_{{t:t+l}},\mathbf{H}_{t},\mathbf{U}_{t}), $}\nonumber
\end{equation}
and find the set of most possible future strategy sequences $\mathbf{\hat{S}}_{{L}}$ (Eq. \ref{eq:h(s_{t})}) through beam search.
Then, we leverage UFP to estimate the future user feedback after using the strategy sequence in $\mathbf{\hat{S}}_{{L}}$. 
Finally, combing the predicted probabilities of the strategy sequences and the user feedback after using them, we obtain the lookahead score $h(s_{t})$ as in Eq. \ref{eq:h(s_{t})}. 
Finally, given $g(s_{t})$ and $h(s_{t})$, the strategy score is obtained as in Eq. \ref{eq:F(s_{t})}.
In the following, we will describe the architectures of SSG and UFP in detail. % architectures respectively and then illustrate how we leverage them to calculate the strategy score during inference. 

\vspace{1mm}\noindent\textbf{Strategy Sequence Generator.}
SSG is developed upon architecture of the Transformer decoder, whose input includes the shifted right strategy sequence $s_{\ge t}$ and the context information, $\mathbf{H}_{t}$ and $\mathbf{U}_{t}$. %Its output at each timestep $l$ ($l$=0, 1, ..., $L-1$) is the predicted strategy distribution $\text{Pr}(s_{{t+l}}|s_{{t:t+l}},\textbf{H}_t,\textbf{U}_t)$. 
Its only difference from the original Transformer decoder is that it adopts the multi-source attention mechanism to selectively focus on both the dialogue history and the user state information. 
Specifically, the shifted right strategy sequence is first fed to a masked multi-head attention layer, %followed by add and normalization,
producing the contextualized strategy sequence representations $\mathbf{P}_t$. 
Then, $\mathbf{P}_t$ interacts with  $\mathbf{H}_t$ and  $\mathbf{U}_t$ respectively, through cross attention layers as:
\begin{align}
    \hat{\mathbf{H}}_t &= \texttt{MH-ATT}(L(\mathbf{P}_t), L(\mathbf{H}_t), L(\mathbf{H}_t)),\nonumber\\
    \hat{\mathbf{U}}_t &= \texttt{MH-ATT}(L(\mathbf{P}_t), L(\mathbf{U}_t), L(\mathbf{U}_t)),\nonumber
\end{align}
where $\texttt{MH-ATT}(\cdot)$ represents the operation of the multi-headed self-attention mechanism. % and $L$($\cdot$) linearly transforms embeddings to form $h$ heads .  
An information fusion layer is utilized to combine them as:
\begin{align}
    \mu &= \text{sigmoid}(\mathbf{W}_{\mu}[\hat{\mathbf{H}}_t; \hat{\mathbf{U}}_t]+\mathbf{b}_{\mu}), \nonumber\\
    \hat{\mathbf{P}}_t  &= \mu \cdot \hat{\mathbf{H}}_t + (1-\mu) \cdot  \hat{\mathbf{U}}_t. \nonumber
\end{align}
where $\mathbf{W}_{\mu}$ and $\mathbf{b}_{\mu}$ are trainable parameters. 

Next, $\hat{\mathbf{P}}_t$ is fed to a connected feed-forward network with a residual connection around the sub-layers, followed by layer normalization. Denoting the resulted representations as $\widetilde{\mathbf{P}}_t$, finally the predicted strategy distribution at  the $l$-th timestep is produced by SSG as:% ($l$=0,1,..,$L$-1)
\begin{equation}
    \text{Pr}(s_{{t+l}}|s_{{t:t+l}}, \mathbf{H}_t, \mathbf{U}_t)=\text{softmax}(\mathbf{W}_s\widetilde{\mathbf{P}}_t+\mathbf{b}_s)\nonumber
\end{equation}
where $\mathbf{W}_{s}$ and $\mathbf{b}_{s}$ are trainable parameters.
To train the SSG, we use the negative log-likelihood of the ground-truth strategy $s_{{t+l}}^{*}$ as its loss function. 
\begin{comment}
\begin{align}
  \mathcal{L}_{s} &= -\sum_{l=
  0}^{L-1} \log \text{Pr}(s_{{t+l}}=s_{{t+l}}^{*}\mid s_{{t:t+l}}^{*}, \mathbf{H}_t, \mathbf{U}_t).\nonumber
\end{align}
\end{comment}

\vspace{1mm}\noindent\textbf{User Feedback Predictor.} 
UFP aims to estimate the future user feedback $f(u_{t}, s_{{t:t+L}})$ after using the strategy sequence $s_{{t:t+L}}$, given the previous user sates. 
First, it encodes the strategy sequence $s_{{t:t+L}}$ with a Transformer encoder. Specifically, we leverage a trainable strategy matrix $\mathbf{E}_s \in \mathbb{R}^{|\mathbb{S}| \times d_{\text{emb}}}$ to represent different types of strategies. Given the strategy sequence $s_{{t:t+L}}$, it is represented as the concatenation of the corresponding strategy vectors based on $\mathbf{E}_s$. Denoting the encoder as $\text{TRS}_{\text{Enc}}$ and its embedding layer as Emb($\cdot$), then we have the resultant representations:
$$\mathbf{B} = \text{TRS}_{\text{Enc}}[\text{Emb}(\texttt{[CLS]};s_{t:t+L})].$$ %, where Emb($\cdot$) represents the operation of the embedding layer that maps the strategies in $s_{t:t+L}$ to their corresponding vectors based on $\mathbf{E}_s$. 
%and $\mathbf{B} \in \mathbb{R}^{(t+L+1)\times d_{emb}}$.
We define the encoded hidden state corresponding to the $\texttt{[CLS]}$ token as $\mathbf{q}_s=\mathbf{B}_0$. %, which will be used later to interact with the user state information. 
Then, $\mathbf{q_s}$ attends to the user state embeddings $\{\mathbf{u}_1, \mathbf{u}_2,...,\mathbf{u}_{t-1}\}$ through an attention layer as in \citet{luong2015effective}, producing the target vector $\widetilde{\mathbf{u}}_f$.
Finally, we obtain the predicted user feedback score  $f(u_{t}, s_{{t:t+L}})$ by passing $\widetilde{\mathbf{u}}_f$ into a single feedforward layer.

%the hidden representations produced by the LSTM through an attention layer as in \citet{luong2015effective}, producing the target vector $\widetilde{\mathbf{u}}_f$.

%Simultaneously, a Long Short-Term Memory (LSTM) \cite{hochreiter1997long} encoder is used to encode the user state embeddings. 
%Then, $\mathbf{q_s}$ attends to user the hidden representations produced by the LSTM through an attention layer as in \citet{luong2015effective}, producing the target vector $\widetilde{\mathbf{u}}_f$. 
%Denoting the hidden representations produced by the LSTM as $\{\overline{\mathbf{u}}_1, \overline{\mathbf{u}}_2,...,\overline{\mathbf{u}}_{t-1}\}$, they are then fed to an attention layer $\widetilde{\mathbf{u}}_f$ through an attention layer as in  \citet{luong2015effective}, using  $\mathbf{q_s}$ as the target hidden state. 
 %obtain the predicted user feedback score $f(u_{t}, s_{{t:t+L}}) = \mathbf{W}_f\widetilde{\mathbf{u}}_f+\mathbf{b}_f\nonumber$, where $\mathbf{W}_f$ and $\mathbf{b}_{f}$ are trainable parameters. 

We leverage the ground-truth user feedback scores annotated in the \textsc{ESConv} dataset as supervision to train the UFP, and use the Mean Square Error (MSE) as its loss function $\mathcal{L}_{f}$. %For training of the user feedback predictor, the negative log-likelihood of the ground-truth strategy $s_{{t+l}}^{*}$ as its loss function:

\subsection{Utterance Decoder} 
Given the user state embeddings $\mathbf{U}_{t}$, the history embeddings $\mathbf{H}_t$, and the selected strategy $s_{t}$, the utterance decoder aims to produce the next utterance $x_{t}$. 
%It is developed upon the backbone of the Transformer decoder. 
Its architecture is the same as that of the strategy sequence generator as shown, except for the input sequence. 
To guide dialogue generation with the selected strategy $s_{t}$, we concatenate the strategy embedding of $s_{t}$ with the embeddings of the shifted right response sequence as the input of the utterance decoder. The negative likelihood of the ground-truth token in the target utterance is used as the generation loss $\mathcal{L}_{g}$. More details on the training procedure are provided in the appendix. 

%\cite{liu2021pre}

==> backup/4_Experiments_2.0.tex <==
\section{Experimental Setup}
\subsection{Dataset} Our experiments are conducted on the \textsc{ESConv} dataset \cite{liu2021towards}. We follow the original division of the \textsc{ESConv} dataset for training, validation and testing. 
%To construct the dataset, they recruited crowdworkers, who had learned the common procedures and strategies for providing emotional support, to converse with volunteers that needed emotion support through an online platform. 
%\textsc{ESConv} contains rich annotation. 
%For example, the supporters were required to annotate the strategy adopted at each turn, and the support-seekers were asked to give feedback every two rounds (on a 5-likert scale, indicating how much their emotional distress is reduced). There are overall 7 kinds of strategies. Each dialogue contains an average of 29.8 utterances, which is much longer than in most dialogue tasks. 

\subsection{Compared Methods}
\subsubsection{Baselines} %Since the task of developing data-driven multi-turn ESC systems is relatively new, our baselines mainly include several systems. The following baselines are implemented to compare with \textsc{MultiESC}. 
\textbf{MoEL} \cite{moel}, \textbf{MIME} \cite{majumder2020mime} and \textbf{EmpDG} \cite{li2020empdg} are three empathetic response generators. MoEL adopts several decoders focusing on different emotion types.
{MIME} follows the architecture of MoEL and adds extra mechanisms to combine the results from different decoders. 
{EmpDG} learns how to generate responses consistent with the user's emotion via an adversarial learning framework. 
%\item \textbf{Sequicity} \cite{lei2018sequicity} incorporates a belief span to model the dialog state to improve generation. We use the support strategy as the belief span to apply it to our task. % and 
%\textbf{DialoGPT-Joint} and \textbf{BlenderBot-Joint} \cite{liu2021towards} are developed on the backbones of DialoGPT \cite{zhang2020dialogpt} and BlenderBot \cite{roller-etal-2021-recipes}, respectively. They prepend a special token, denoting the predicted support strategy, before the generated utterance. % to generate content conditioned on a predicted strategy. 

\noindent\textbf{DialoGPT-Joint}, \textbf{BlenderBot-Joint} \cite{liu2021towards}, \textbf{MISC} \cite{tu2022misc} and \textbf{GLHG} \cite{peng2022control} are four state-of-the-art models on the ESConv dataset. {DialoGPT-Joint} and {BlenderBot-Joint} are developed based on DialoGPT \cite{zhang2020dialogpt} and BlenderBot \cite{roller-etal-2021-recipes}, respectively. They prepend a special token denoting the predicted strategy before the generated utterance. MISC predicts the strategy distribution using a Transformer encoder to guide the response generation. %They also enhance context encoding with commonsense knowledge. % and uses the predicted strategy distribution to guide the response generation. It predicts the strategy distribution using a vanilla Transformer encoder. 
GLHG adopts a graph neural network to model the relationships between the user's emotion causes, intentions and the dialogue history. % for emotional support dialogue generation. 

\subsubsection{Ablations of MultiESC} 
%For ablation study, we compare \textsc{MultiESC} with its following variants. 
\noindent\textbf{MultiESC \emph{w/o} cause} does not incorporate emotion cause extraction for user state modeling. 

\noindent\textbf{MultiESC \emph{w/o} emotion} does not incorporate emotion embeddings in the user state modeling module.

\noindent\textbf{MultiESC \emph{w/o} strategy} directly generates utterances without first predicting the used strategy.

\noindent\textbf{MultiESC \emph{w/o} lookahead} conducts strategy planning without the lookahead heuristics that estimate the long-term user feedback scores. 

\subsection{Implementation Details.}
We initialize the parameter of the dialogue encoder and the utterance decoder of MultiESC with the BART-small \cite{lewis2020bart} model from the HuggingFace Transformer library \cite{Wolf2019huggingface}. 
The maximum length of the input sequence for the dialogue encoder is $N$=$512$. 
There are $n_{\text{emo}}$=$65$ types of emotion vectors, with $n_\text{V}$=$n_\text{A}$=8. 
In the strategy planning module, we set $\lambda$ as 0.3; we experiment with $L$ between 2-5 and find that $L$=2 performs slightly better. 
The beam size is set to beam-$k$=6. 
%The dimensions of all the hidden embeddings are $d_{\text{emb}}$=$768$. 
Since the codes of MISC and GLHG were not released, we directly refer to the results reported in their original papers. For the other compared models, we directly use their released codes to conduct our experiments. 
%We use the small versions of DialoGPT and BlenderBot. 
%AdamW \cite{Losh2017AdamW} is used as optimizer; its initial learning rate is set to be $5$$\times$$10^{-5}$. % and adaptively decays during training. 
%The batch size is set to 32.  
Each model is trained up to 10 epochs, and the checkpoints that achieves the best BLEU scores on the validation set are used for evaluation. 

\subsection{Evaluation Metrics}
\paragraph{Automatic Evaluation of Generation Quality}
%We adopt the following automatic metrics: perplexity (\textbf{PPL}), BLEU-1/2/3/4 (\textbf{B-1/2/3/4}) \cite{papineni2002bleu}, ROUGE-L (\textbf{R-L}) \cite{lin2004rouge}, METEOR (\textbf{MET}) \cite{Lavie2007Meteor}, CIDEr (\textbf{CID}) \cite{vedantam2015cider}. 
To evaluate the generation quality, we adopt the following automatic metrics: perplexity (\textbf{PPL}), BLEU-1/2/3/4 (\textbf{B-1/2/3/4}), which measure the n-gram precision; ROUGE-L (\textbf{R-L}) \cite{lin2004rouge}, measuring the recall of longest common subsequences; METEOR (\textbf{MET}) \cite{Lavie2007Meteor}, which further considers stem match, or synonymy match; \textbf{CIDEr} \cite{vedantam2015cider}, measuring the similarity between TF-IDF weighted n-grams (i.e., the words that frequently appear in many utterances contribute less to the score). 


\paragraph{Human Interactive Evaluation}
For human interactive evaluation, we recruit four workers from a third-party company to chat with the models. We randomly sample 100 test instances. 
The evaluators are asked to act as the support seekers in these test instances by learning their situations, and simulate their process of seeking emotional support by chatting with the models. 
Given MultiESC and a compared model, the recruited workers are asked to choose which one performs better (or select \emph{tie}). %The compared models were randomly ordered to avoid exposure bias.
Following \citet{liu2021towards}, we adopt the following metrics in human evaluation: 
    (1) \textbf{Fluency}: which model generates more fluent and understandable responses; 
    (2) \textbf{Empathy}: which model has more appropriate emotion reactions, such as warmth, compassion and concern; 
    (3) \textbf{Identification}: which model explore the user's situation more effectively to identify the problem; 
    (4) \textbf{Suggestion}: which model gives more helpful suggestion to the user; 
    (5) \textbf{Overall}: which model is better capable of providing emotional support overall. 

\paragraph{Automatic Evaluation of Strategy Planning} To evaluate the capabilty of strategy planning, 
we use accuracy (\textbf{Acc}), Weighted F1 (\textbf{W-F1}), and \textbf{Feedback} as the evaluation metrics. 
Accuracy and weighted F1 directly compare the prediction results with ground-truth labels. Accuracy reflects the overall performance, and weighted F1 measures the weighted average of F1 scores on different class while taking the class imbalance into account. \emph{feedback} simulates the user feedback score that would be given if the predicted strategy is adopted. It is implemented with an automatic user feedback predictor as illustrated in Sec. \ref{sec:strategyMultiESC}. 

\section{Experimental Results}
\input{Table/1-generation_auto}
\subsection{Automatic Evaluation of Generation Quality} \label{sec:eval_generation}
%We first compare the generation results of \textsc{MultiESC} with those of the baseline models, using both automatic and human evaluation. 
\paragraph{Comparison with Baselines} 
%where the top three rows are the baselines that focus on empathetic responding, while the middle three also take strategy planning into account. 
Table \ref{tbl:generation_auto} shows the automatic evaluation results on generation quality. 
We can see that \textsc{MultiESC} performs significantly better than the baseline models in all the automatic metrics, demonstrating the effectiveness of our proposed method. %44.67\% 15.07\% 10.43\% 46.02\%
It performs especially well in terms of the CIDEr metric, %Another major finding is that the models that consider strategy selection/planning achieve remarkably higher
which demonstrates that it is more capable of including key information in the responses, catering to particular situations of users. %, when taking strategy planning into account. 
In comparison, the three empathetic generators (MoEL, MIME and EmpDG) achieve significantly worse perplexity and the CIDEr score than the other models. 
Through analysis, we found that theses empathetic generators tend to include content that commonly appear in many samples (e.g. ``I'm sorry to hear that'', ``that's horrible!''). This is probably because they only focus on how to generate responses that can display understanding of the user's emotion, which is not sufficient for providing emotional support.  %These results illustrate the importance of strategy planning in ESC. 


%\input{backup/2-generation_human_backup}


\paragraph{Ablation Study}% \input{Table/5-user_state_modeling}
We also conduct ablation studies to analyze the effects of different components on the downstream generation in \textsc{MultiESC}. 
The results are shown in the lower part of Table \ref{tbl:generation_auto}. 
We can see that the ablation of every component can all cause a drop in the performance of downstream generation, demonstrating the indispensability of each part. 
%Note that if the improvement brought by the strategy planning module in these automatic metric cannot sufficiently illustrate the importance of strategy planning . %predicted strategy is different from the ground truth, the generated response will be much different from the reference response.

\input{Table/2-generation_human}

\subsection{Human Interactive Evaluation}  % on a particular test instance. 
As shown in Table \ref{tbl:generation_human}, we can see that \textsc{MultiESC} perform significantly better than MoEL and Sequicity in all the human evaluation metrics. 
It is also better than BlenderBot in most metrics except fluency. This is probably because BlenderBot is pretrained on a large-scale of dialogue data, while \textsc{MultiESC} does not. 
Among the three baselines, the performance gap between MoEL and \textsc{MultiESC} is largest, which again demonstrates that providing emotional support requires more skills than expressing empathy. 
Among the four fine-grained metrics, \textsc{MultiESC} perform especially well in terms of identification and suggestion. %, demonstrating its better capability of identifying the user's situations and providing helpful suggestions. 
Compared with the other two metrics,  identification and suggestion are more closely related to strategy planning; the model needs strategic planning on how to gradually inquire about the user's problem and provide appropriate suggestions accordingly. 
These results to some extent reflect the competitive ability of strategy planning in \textsc{MultiESC}. 

Analysis of Strategy-Enhanced Generation. %\red{Add an automatic evaluation of ablation study for Strategy-Enhanced Generation as Table \ref{tbl:user_state}.}
To test whether our proposed method of strategy planning enhances the downstream generation, we conduct human evaluation to compare \textsc{MultiESC} with its two ablated variants. 


\subsection{Analysis of Strategy Planning}
\input{Table/3-strategy_acc} 
%\input{Table/4-strategy_enhanced}
%\paragraph{Evaluation of Next Strategy Selection} 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figure/plot.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
We evaluate the strategy planning module of MultiESC individually, and compare it with the three baselinse that are capable of strategy planning (DialoGPT-Joint, BlenderBot-Joint, MISC). The results are shown in Table \ref{tbl:strategy_acc}. We can see that our full model performs the best in all three metrics, especially in the feedback metric. It demonstrates that our model is able to select appropriate strategies that more effectively comfort the users. The full model's superior performance over the ablated version without lookahead heuristics also illustrates the necessity of long-term lookahead planning. 
%Its difference from the UFP implemented in the MultiESC system is that it aims to predict feedback after using one next strategy instead of a strategy sequence (which contains multiple strategies). 
%The evaluation metrics include \textbf{accuracy} and \textbf{weighted F1}, which compare prediction results with ground-truth labels. Accuracy reflects the overall performance, and weighted F1 measures the weighted average of F1 scores on different class while taking the class imbalance into account. Considering that multiple strategies can be all appropriate given the same dialog context, we incorporate the user feedback score (\textbf{feedback}) as another metric. We implement an automatic user feedback predictor, whose architecture is the same as described in Sec. \ref{sec:strategyMultiESC}. Its difference from the UFP implemented in the MultiESC system is that it aims to predict feedback after using one next strategy instead of a strategy sequence (which contains multiple strategies). 
%To further assess the system's capability of providing emotional support, we recruit three annotators to directly conduct pairwise comparison between \textsc{MultiESC} and three competitive baselines (MoEL, Sequicity, and BlenderBot) respectively. We randomly select 100 dialogues in the test set and evaluate the models' performance on these samples. 
%baseline models for predicting the support strategy used in the next turn, which are \textbf{BERT} \cite{devlin2018bert} and \textbf{HED}. BERT takes the concatenation of dialogue history as input to predict the strategy, while HED is an hierarchical encoder that first encodes every utterance locally with a Transformer and then globally combine them through an LSTM. 
%Besides, we observe that the three baselines that jointly learn strategy selection and generation (Sequicity, DialoGPT, and BlenderBot) perform significantly worse than \textsc{MultiESC}.


\begin{comment}

\paragraph{Analysis of Strategy Distribution at Different Conversation Stages} 
\input{Table/6-strategy distribution}
While the selection of strategies should be flexibly adjusted to the user's need and the dialogue context,  psychological guidelines have suggested ordered procedures for providing emotional support \cite{hill2009helping}, where some strategies are advised to be frequently used in the early stage (e.g. \emph{Question}) and some in the late stage (e.g. \emph{Providing Suggestions}). 
To analyze if the models also learn such strategy selection patterns, we report the distribution of strategies at different conversation phases.  
Specifically, we split the conversation into five stages; for a conversation with $L$ utterances, suppose that the $k$-th ($1\le k \le L$) utterance is from the supporter and adopts the strategy $s_k$, we say that this strategy is located at the conversation stage $\lceil 5k/L \rceil $.
Then, for all the conversations in the dataset, we respectively compute the distribution of the ground-truth strategies at each stage and those predicted by BERT and \textsc{MultiESC}, which is presented in Fig. \ref{fig:strategy_distribution}.
We can see that the strategies that \textsc{MultiESC} adopted have a very similar distribution compared with the truth distribution, demonstrating that it has effectively learned the emotional support procedures as adopted by human supporters. \blue{In comparison,}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{Figure/strategy_distribution.png}
    \caption{The distribution of the ground-truth strategies and those predicted by BERT and \textsc{MUltiESC}  at different conversation stages.}
    \label{fig:strategy_distribution}
\end{figure}
\end{comment}


